JNV Corpus: A Corpus of Japanese Nonverbal Vocalizations with Diverse Phrases and Emotions

We present JNV (Japanese Nonverbal Vocalizations) corpus, a corpus of Japanese nonverbal vocalizations (NVs) with diverse phrases and emotions. Existing Japanese NV corpora lack phrase or emotion diversity, which makes it difficult to analyze NVs and support downstream tasks like emotion recognition. We first propose a corpus-design method that contains two phases: (1) collecting NVs phrases based on crowd-sourcing; (2) recording NVs by stimulating speakers with emotional scenarios. We then collect $420$ audio clips from $4$ speakers that cover $6$ emotions based on the proposed method. Results of comprehensive objective and subjective experiments demonstrate that the collected NVs have high emotion recognizability and authenticity that are comparable to previous corpora of English NVs. Additionally, we analyze the distributions of vowel types in Japanese NVs. To our best knowledge, JNV is currently the largest Japanese NVs corpus in terms of phrase and emotion diversities.

==> tables/dataset.tex <==
\begin{table}[t]
    \centering
    \caption{Statistics of JNV. Ang=Angry; Disg=Disgust; Hap=Happy; Surp=Surprise.}
    \vspace{1mm}
    \footnotesize
    \begin{tabular}{ccccc}
    \hline
     & \makecell[cc]{Phrases\\(reg.)} & \makecell[cc]{Phrases\\(free)} & Dur. (s) & Avg. dur. (s) \\
     \hline
    Ang   & $14$   & $3$ & $61.3$  & $0.9$   \\
    Disg  & $10$   & $3$ & $61.4$  & $1.1$  \\
    Fear  & $10$   & $3$ & $44.4$    & $0.9$ \\
    Hap  & $16$    & $3$ & $75.3$  & $1.0$  \\
    Sad  & $7$   & $3$  & $55.9$  & $1.4$ \\
    Surp & $30$  & $3$ & $108.6$ & $0.8$ \\
    $\sum$ & $87$& $18$& $406.9$ & -- \\
    \hline
\end{tabular}
\end{table}

==> tables/sub_rating.tex <==
\begin{table}[t]
    \centering
    \caption{Results of the rating evaluation (scaled to $0-100$) and the derived accuracy ($\%$). \textbf{Bold} indicates the best scores of each emotion. Ang=Angry; Disg=Disgust; Hap=Happy; Surp=Surprise.}
    \vspace{1mm}
    %\small
    \begin{tabular}{cccccccc}
    \hline
    \multirow{2}{*}{Emotion} & \multicolumn{6}{c}{Rating} & \multirow{2}{*}{\makecell[c]{Derived \\accuracy}}\\
    \cline{2-7}
    & Ang & Disg & Fear & Hap & Sad & Surp & \\
    \hline
    Ang & $\mathbf{71.3}$ & $35.7$ & $28.7$ &$11.4$ &$23.1$ &$31.0$ &$88.2$ \\
    Disg  & $37.8$ & $\mathbf{75.1}$ & $51.9$ & $9.9$ & $38.5$ &$39.0$ &$77.8$ \\
    Fear  & $24.4$ &$50.4$ &$\mathbf{68.4}$ &$29.0$ &$38.0$ &$66.0$ &$50.0$ \\
    Hap  & $11.4$&$9.1$ &$12.4$ &$\mathbf{69.5}$ &$10.4$ &$23.0$ &$86.8$ \\
    Sad  &$30.2$ &$45.3$ &$49.3$ &$13.8$ &$\mathbf{66.9}$ &$29.4$ &$52.5$ \\
    Surp  &$30.4$ &$29.8$ &$42.2$ &$41.5$ &$24.1$ &$\mathbf{57.5}$ &$53.0$ \\
    \hline
    \end{tabular}
    \label{tab:rating}
\end{table}
